LVIC: Multi-modality segmentation by Lifting Visual Info as Cue

Multi-modality fusion is proven an effective method for 3d perception for autonomous driving. However, most current multi-modality fusion pipelines for LiDAR semantic segmentation have complicated fusion mechanisms. Point painting is a quite straight forward method which directly bind LiDAR points with visual information. Unfortunately, previous point painting like methods suffer from projection error between camera and LiDAR. In our experiments, we find that this projection error is the devil in point painting. As a result of that, we propose a depth aware point painting mechanism, which significantly boosts the multi-modality fusion. Apart from that, we take a deeper look at the desired visual feature for LiDAR to operate semantic segmentation. By Lifting Visual Information as Cue, LVIC ranks 1st on nuScenes LiDAR semantic segmentation benchmark. Our experiments show the robustness and effectiveness. Codes would be make publicly available soon.

==> exp.tex <==
\begin{figure*}[htbp]
\centering     

\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/32.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/34.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/58.jpg}}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``stop vehicle next to the man with a wheelchair."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``bob is waiting in the car on the left side of the road. i need to pick him up. make a you-turn when safely able to do so."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``that is my wife. stop next to her."
\end{minipage}

\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/82.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/103.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/119.jpg}}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``watch out for that guy, i think he might try to cross the street. better slow down."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``take a left turn after that silver car parked on the left."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``park just passed where that dog is."
\end{minipage}

\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/198.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/229.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/2379.jpg}}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``par in front of that old truck on the other side of the road."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``pull up next to that officer standing more on the road than the other one. i want to talk to him."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``let the car on the left overtake you."
\end{minipage}

\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/2366.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/251.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/101.jpg}}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``i see my friend mark. stop here for a moment"
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``pull up next to the guy wearing the safty vest so i can talk to him"
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``park behind the car infront of the mail truck"
\end{minipage}


\caption{\textbf{Visualization results on Talk2Car.} The green bounding box in the image corresponds to the ground truth, while the red bounding box represents the output generated by our model. The instruction corresponding to the image is provided below.}
\label{fig:qualitative}
\end{figure*}
